Local Unitarity: cutting raised propagators and localising renormalisation

The Local Unitarity (LU) representation of differential cross-sections locally realises the cancellations of infrared singularities predicted by the Kinoshita-Lee-Nauenberg theorem. In this work we solve the two remaining challenges to enable practical higher-loop computations within the LU formalism. The first concerns the generalisation of the LU representation to graphs with raised propagators. The solution to this problem results in a generalisation of distributional Cutkosky rules. The second concerns the regularisation of ultraviolet and spurious soft singularities, solved using a fully automated and local renormalisation procedure based on Bogoliubov's R-operation. We detail an all-order construction for the hybrid $\overline{\text{MS}}$ and On-Shell scheme whose only analytic input is single-scale vacuum diagrams. Using this novel technology, we provide (semi-)inclusive results for two multi-leg processes at NLO, study limits of individual supergraphs up to N3LO and present the first physical NNLO cross-sections computed fully numerically in momentum-space, namely for the processes $\gamma^* \rightarrow j j$ and $\gamma^* \rightarrow t \bar{t}$.

==> test.tex <==
\section{Local UV subtraction and automatic renormalization}
In Local Unitarity, the amplitudes on either side of the Cutkosky cut may have remaining loops. Generally, these loop amplitudes have remaining ultraviolet divergences. To be able to Monte Carlo integrate them, we will have to introduce local counterterms to subtract these divergences. The local counterterms should not introduce additional infrared singularities and ideally align with a renormalization scheme. For renormalization scheme transitions, the counterterms should be straightforward to integrate analytically. In this chapter we will construct local counterterms through the $R$- procedure, and perform a renormalization scheme transition to $\overline{MS}$. The entire procedure is automated in a FORM code.

The $R$-operation~\cite{Bogoliubov:1957gp,Zimmermann:1969jj,Herzog:2017jgk} enumerates all divergent loop cycles and its combinations thereof and subtracts them in a fashion such that overlapping divergences are also properly subtracted. Since the divergent components are described in terms of cycles and expansions in momenta, it can be applied to construct local counterterms.

\subsection{Local counterterms}
The procedure to determine all divergent components starts with the construction of all 1PI subgraphs. To determine if these subgraphs are divergent, we sum the mass dimension of all the edges and vertices in the subgraph (i.e., a quark propagator has mass dimension -1, a triple gluon vertex +1). This quantity is referred to as the \emph{degree of divergence} (dod) and if it is greater than or equal to 0, the graph is ultraviolet divergent.

\begin{figure}
\centering
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{feynman}
\vertex (a3);
\vertex[right=1cm of a3] (a4);
\vertex[right=1cm of a4] (a5);
\vertex[right=1cm of a5] (a6);
\vertex[right=1.5cm of a6] (bb6);
\vertex[right=2cm of a6] (a7);
\vertex[right=1cm of a7] (a8);
\vertex[right=1cm of a8] (a9);
\vertex[right=1cm of a9] (a10);

\vertex[below=0.5cm of a8] (b1);

\vertex[above=of bb6] (c1);
\vertex[above=1cm of c1] (c3);
\vertex at ($(c1)!0.5!(c3) - (1cm, 0)$) (c2);
\vertex[right=2cm of c2] (c4);

\diagram* {
{
(a4) -- (a5) -- [edge label=${10}$] (a6) -- [edge label=${6}$] (a7) -- [edge label=${11}$] (a8) -- [edge label=${12}$] (a9) -- (a10),
},

(c1) -- [out=180,in=-90, edge label={$2$}] (c2) -- [out=90,in=180,edge label={$1$}] (c3) -- [out=0, in=90,edge label={$4$}] (c4) -- [out=-90,in=0,edge label={$5$}] (c1),
(a9) -- [boson, bend right, edge label={$9$}] (c4),
(c1) -- [boson, edge label={$3$}] (c3),
(a5) -- [boson, bend left, edge label={$8$}] (c2),
(a6) -- [boson, out=-90, in=-90, edge label={$7$}] (a7),
(a8) -- [boson] (b1),
};
\end{feynman}
\end{tikzpicture}
\caption{Example graph with nested ultraviolet divergences. Its UV spinneys is $\{\gamma_{6 7}, \gamma_{1 2 3}, \gamma_{3 4 5}, \gamma_{1 2 3 4 5}, \gamma_{1 \ldots 12}\}$.}
\label{fig:uvexample}
\end{figure}

We apply the procedure sketched above to the amplitude in fig.~\ref{fig:uvexample}. The UV divergent subgraphs $\gamma$ are denoted using their edge numbers. The vertices at the endpoints of the edges are understood to be part of the subgraph. The UV divergent subgraphs are $\{\gamma_{6 7}, \gamma_{1 2 3}, \gamma_{3 4 5}, \gamma_{1 2 3 4 5}, \gamma_{1 \ldots 12}\}$. The degree of divergence of $\gamma_{6 7}$ is 1 (linear), of $\gamma_{1 2 3}$ and $\gamma_{3 4 5}$ is 0 (logarithmic), of $\gamma_{1 2 3 4 5}$ is 2 (quadratic), and of $\gamma_{1 \ldots 12}$ is 0.

From these UV divergent subgraphs, we can construct the \emph{spinney}, by taking the power set of all UV divergent subgraphs and keeping only the sets where any two subgraphs are disjunct, i.e., sharing no edge or vertex. We obtain the following spinneys:
\begin{equation}
\{
\{\},
\{\gamma_{6 7}\}, \{\gamma_{1 2 3}\}, \{\gamma_{3 4 5}\}, \{\gamma_{1 2 3 4 5}\}, \{\gamma_{1\ldots12}\},\{\gamma_{1 2 3}, \gamma_{6 7}\}, \{\gamma_{1 2 3}, \gamma_{6 7}\}, \{\gamma_{1 2 3 4 5}, \gamma_{6 7}\}
\}
\end{equation}
A notable spinney that is absent is $\{\{\gamma_{1 2 3}\}, \{\gamma_{3 4 5}\}\}$, since these two subgraphs overlap. The subgraphs $\gamma_{1 2 3 4 5}$ and $\gamma_{1\ldots12}$ have subdivergences.

Using these components, we now present the $R$-procedure~\cite{Bogoliubov:1957gp} that yields a finite integral:
\begin{equation}
R(\Gamma) = \sum_{S \subseteq \Gamma} \prod_{\gamma \in S} Z(\gamma) * \Gamma / S,\quad Z(\Gamma) = -K\left(\sum_{S \subsetneq \Gamma} \prod_{\gamma \in S} Z(\gamma) * \Gamma / S\right)
\end{equation}
where $S$ are the spinneys of $\Gamma$.
$Z(\gamma)$ is the local UV counterterm operator which subtracts subdivergences and has $Z(\emptyset)$ = 1. It is a polynomial in the external momenta and internal masses~\cite{Bogoliubov:1957gp}. $\Gamma / S$ is the \emph{remaining graph}: the graph where the UV divergent graphs have been shrunk to a point, into which the value of the counterterm will be inserted. $K$ is a scheme-dependent renormalization operator that should yield the divergent part of the integral expressed in some regulator. The minus sign in the definition of $Z(\Gamma)$ takes care of the proper subtraction of overlapping divergences through an inclusion-exclusion principle. The nested $R$-operation can also be written in terms of the BHPZ forest formula~\cite{Zimmermann:1969jj,Hepp:1966eg}, but in this language it is hard to express the nesting and iteration of the $K$-operator, which is critical for a proper scheme definition. It is also important that the Feynman rules are not substituted before the $R$-operation is applied, since this invalidates the power counting and it does not commute with the $K$-operator in general~\cite{Caswell:1981ek,Herzog:2017bjx}.


For the example graph in fig.~\ref{fig:uvexample}, the spinney $\{\gamma_{1 2 3 4 5},\gamma_{6 7}\}$ yields:
\begin{align}
+ K(\gamma_{6 7}) K(\gamma_{1 2 3 4 5} - K(\gamma_{1 2 3}) * \gamma_{4 5} - K(\gamma_{3 4 5}) * \gamma_{1 2} ) * \gamma_{8 \ldots 12} \;.
\end{align}

In order to obtain a local counterterm, $K(\gamma)$ should be a local approximant of the UV behaviour of $\gamma$, which is satisfied when $K$ acts as a Taylor expansion in the limit of the loop momentum going to infinity. Equivalently, we can take the limit of all external momenta and masses in the subgraph going to zero. The depth of the expansion equals the degree of divergence. This choice of $K$ relates to a momentum-space subtraction scheme. In this scheme, the UV counterterm $Z(\gamma)$ is a massless tensor vacuum graph. For analytic computation such an object is convenient\cite{Herzog:2017bjx}, but it could generate spurious IR divergences. Instead, we expand each propagator as follows:
\begin{equation}
T\left(\frac{1}{(k+p)^2-m^2}\right) = \lim_{\lambda \rightarrow 0} \frac{1}{k^2 -m_{UV}^2 +2\lambda k \cdot p + \lambda^2 - \lambda^2 m^2}
\end{equation}
where $m_{UV}$ is a UV mass that is introduced as a regulator for the infrared behaviour. Importantly, such an infrared rearrangement\cite{Lowenstein:1974qt,Vladimirov:1979zm} does not spoil the local cancellation of the counterterm.

We write $K(\gamma)=T_{\text{dod}}(\gamma)$, where $\text{dod}$ is the degree of divergence of $\gamma$. For our example spinney we obtain:
\begin{align}
+ T_1(\gamma_{6 7}) T_2(\gamma_{1 2 3 4 5} - T_0(\gamma_{1 2 3}) * \gamma_{4 5} - T_0(\gamma_{3 4 5}) * \gamma_{1 2} ) * \gamma_{8 \ldots 12} \;.
\end{align}
The Taylor expansion yields a tensor graph in terms of the polynomial in the external momenta of the subgraph and the operator $*$ signifies that the tensor structure is multiply into the remaining graph at the vertex where the UV subgraph has been shrunk. If this graph was nested inside a $K$, the expansion over all the masses as part of the $K$-operation will also expand over the $m_{UV}$ factors in the numerator stemming from the Taylor expansion of the UV subgraph.

In order to perform the Taylor expansion in the external momenta, a change of basis has to be performed on every term of the form $T(\gamma_1)*\gamma_2$, such that every $n$-loop UV subgraph has exactly $n$ independent momenta. We show the spinney $T(\gamma_{1 2 3})*\gamma_{4 5}$ as an example:
\begin{align}
\begin{tikzpicture}[baseline=(c2.center)]
\tikzstyle{every node}=[font=\small]
\begin{feynman}
\vertex (c1);
\vertex[above=1cm of c1] (c3);
\vertex at ($(c1)!0.5!(c3) - (1cm, 0)$) (c2);
\vertex[right=2cm of c2] (c4);
\vertex[left=1cm of c2] (d1);
\vertex[right=1cm of c4] (d2);
\diagram* {
(c1) -- [out=180,in=-90, edge label={$k+p$}] (c2) -- [out=90,in=180,edge label={$k$}] (c3) -- [out=0, in=90,edge label={$k+l$}] (c4) -- [out=-90,in=0,edge label={$k+l+p$}] (c1),
(d2) -- [boson, edge label'={$p$}] (c4),
(c1) -- [boson, edge label={$l$}] (c3),
(d1) -- [boson, edge label={$p$}] (c2),
};
\end{feynman}
\end{tikzpicture}
& \rightarrow
T\left(
\begin{tikzpicture}[baseline=(c2.center)]
\tikzstyle{every node}=[font=\small]
\begin{feynman}
\vertex (c1);
\vertex[above=1cm of c1] (c3);
\vertex at ($(c1)!0.5!(c3) - (1cm, 0)$) (c2);
\vertex[right=2cm of c2] (c4);
\vertex[left=1cm of c2] (d1);
\vertex[right=1cm of c4] (d2);
\vertex[right=0.5cm of c3] (e1);
\vertex[right=0.5cm of c1] (e2);
\diagram* {
(e2) -- [edge label=$k+l+p$,near start] (c1) -- [edge label=$k+p$] (c2) -- [edge label=$k$] (c3) -- [edge label=$k+l$] (e1),
(c1) -- [boson, edge label={$l$}] (c3),
(d1) -- [boson, edge label={$p$}] (c2),
};
\end{feynman}
\end{tikzpicture}
\right)
*
\begin{tikzpicture}[baseline=(c2.center)]
\tikzstyle{every node}=[font=\small]
\begin{feynman}
\vertex (c1);
\vertex[above=1cm of c1] (c3);
\vertex[crossed dot] at ($(c1)!0.5!(c3) - (1cm, 0)$) (c2) {};
\vertex[right=2cm of c2] (c4);
\vertex[left=1cm of c2] (d1);
\vertex[right=1cm of c4] (d2);
\vertex[right=0.5cm of c3] (e1);
\vertex[right=0.5cm of c1] (e2);
\diagram* {
(c4) -- [bend left, edge label=$k+l+p$] (c2) -- [bend left,edge label=$k+l$] (c4),
(d1) -- [boson, edge label={$p$}] (c2),
(d2) -- [boson, edge label'={$p$}] (c4),
};
\end{feynman}
\end{tikzpicture}
\\&\rightarrow
T\left(
\begin{tikzpicture}[baseline=(c2.center)]
\tikzstyle{every node}=[font=\small]
\begin{feynman}
\vertex (c1);
\vertex[above=1cm of c1] (c3);
\vertex at ($(c1)!0.5!(c3) - (1cm, 0)$) (c2);
\vertex[right=2cm of c2] (c4);
\vertex[left=1cm of c2] (d1);
\vertex[right=1cm of c4] (d2);
\vertex[right=0.5cm of c3] (e1);
\vertex[right=0.5cm of c1] (e2);
\diagram* {
(e2) -- [edge label=$c_1+c_2+p$] (c1) -- [edge label=$c_1+p$] (c2) -- [edge label=$c_1$] (c3) -- [edge label=$c_2$] (e1),
(c1) -- [boson, edge label'={$c_1 + c_2$}] (c3),
(d1) -- [boson, edge label={$p$}] (c2),
};
\end{feynman}
\end{tikzpicture}
\right)
*
\begin{tikzpicture}[baseline=(c2.center)]
\tikzstyle{every node}=[font=\small]
\begin{feynman}
\vertex (c1);
\vertex[above=1cm of c1] (c3);
\vertex[crossed dot] at ($(c1)!0.5!(c3) - (1cm, 0)$) (c2) {};
\vertex[right=2cm of c2] (c4);
\vertex[left=1cm of c2] (d1);
\vertex[right=1cm of c4] (d2);
\vertex[right=0.5cm of c3] (e1);
\vertex[right=0.5cm of c1] (e2);
\diagram* {
(c4) -- [bend left, edge label=$c_2 + p$] (c2) -- [bend left,edge label=$c_2$] (c4),
(d1) -- [boson, edge label={$p$}] (c2),
(d2) -- [boson, edge label'={$p$}] (c4),
};
\end{feynman}
\end{tikzpicture}
\end{align}
where on the last line we transformed into the expansion basis $c_1=k, c_2=k+l$.
After performing the expansion, all terms are transformed back to the original basis. In order to have local UV cancellations in this basis, an expansion basis has to be chosen consistently between the terms. An example of a bad basis for the example above would be $c_1=k+p, c_2=k+l$ if one had selected the basis $c_1=k,c_2=l$ for $\gamma_{1 2 3 4 5}$, as this leads to miscancellations in the double limit.
A simple way to achieve this, is to make sure that the basis transformation does not involve shifts. Note that in some higher-loop cases a UV subgraph may have no propagators that are shiftless.

For Local Unitarity, it is also important that the same basis momenta are chosen between Cutkosky cuts that share the same UV subgraph, since the counterterms of the subgraph should be exactly the same in order to have IR cancellations. This can be achieved by selecting preferred momenta for subgraphs at the supergraph level.

\subsection{Scheme conversion to $\overline{MS}$}

The procedure outlined above produces a locally UV-finite expression for amplitudes as well as for Local Unitarity, and produces a renormalized result in a momentum subtraction scheme. For many computations and for comparison with the literature it is often convenient to produce results in $\overline{MS}$. In $\overline{MS}$ the $K$-operation is not a Taylor expansion, but is defined as taking the pole part of the Laurent series in the dimensional regulator $\epsilon$, for dimension $D=4-2 \epsilon$. We will now construct the scheme transition terms.

The arguments of $K$ in the $R$-operation are a graph minus its subdivergences. The poles of this quantity are polynomial in the external momenta and masses~\cite{Bogoliubov:1957gp}. As a consequence, the Taylor expansion operator of the momentum subtraction scheme $K$ leaves the poles invariant. Thus we obtain:
\begin{equation}
K^{\overline{MS}}(\Gamma) = K^{\overline{MS}}([K(\Gamma)])
\end{equation}
where $[\Gamma]$ denotes the integrated graph $\Gamma$ in dimensional regularisation.

Then we see that we can rewrite the $\overline{MS}$ $K$-operation into a local $K$-operation and a finite quantity:
\begin{equation}
K^{\overline{MS}}(\Gamma) = K^{\overline{MS}}(K[\Gamma]) = K^{\overline{MS}}(K[\Gamma]) + K(\Gamma) - [K(\Gamma)] =
K(\Gamma) + (1-K^{\overline{MS}})*[K(\Gamma)]
\end{equation}
where $(1-K^{\overline{MS}})$ removes the pole part in $\epsilon$ of the analytic computation of $K(\Gamma)$.

Thus, adding an integrated level modification $(1-K^{\overline{MS}})*[K(\Gamma)]$ to the local counterterm operator produces $\overline{MS}$ results. Since the loop momenta of the UV subgraph have been integrated in this term, the new term cannot directly be added to the numerical integration without proper normalization of these integrated dimensions. We multiply the $\overline{MS}$ conversion term with the finite integrand
\begin{equation}
\frac{2 i (4 \pi)^2 m_{UV}^2}{(k^2-m_{UV}^2)^3} \;,
\end{equation}
which integrates to 1, for every integrated loop variable $k$.

In conclusion, with this added factor we will obtain a locally finite integrand that integrates to $\overline{MS}$.

\cmtBR{mention other schemes such as the on-shell scheme?}

\subsection{Computation of the integrated counterterms}
The $\overline{MS}$ conversion factor involves the analytic computation of single-scale massive tensor vacuum graphs. Within our implementation we have full support for these computation up to and including three-loop amplitudes. In principle this can be extended to four loops~\cite{Pikelner:2017tgv}. Below we sketch the construction of our automated setup.

The first step is to tensor reduce the analytic integrand. Since the integral is a vacuum bubble, all tensor structures reduce to combinations of the metric. For example:
\begin{equation}
\Gamma^{\mu \nu} = A g^{\mu \nu} = \frac{\Gamma^{\alpha \alpha}}{D} g^{\mu \nu}
\end{equation}
With increasing tensor rank, the number of possible metric structures $n$ grows exponentially (rank 6 gives $n=15$, rank 8 gives $n=105$). A naive tensor reduction algorithm would have to solve an $n \cross n$ linear system, which is slow for high rank. An improved algorithm that exploits the underlying symmetry group and symmetries of the momenta that the indices belong to was derived in ref.~\cite{Ruijl:2018poj} and is used in our implementation.

All up to three-loop vacuum bubbles are subsets of only the following three topologies:
\begin{equation}
\begin{tikzpicture}
\begin{feynman}

\tikzfeynmanset{every vertex={empty dot,minimum size=0mm}}
\vertex (a1);

\vertex[right=1cm of a1] (a3);

\tikzfeynmanset{every vertex={empty dot,minimum size=0mm}}

\vertex[right=0.5cm of a1] (a2);
\vertex[above=0.5cm of a2] (a4);
\vertex[below=0.5cm of a2] (a5);

\vertex[left=0.433cm of a2] (b1);
\vertex[left=0.433cm of a2] (b2);

\tikzfeynmanset{every vertex={dot,minimum size=0.8mm}}
\vertex[below right=0.71cm of a1] (b3);


\diagram*[large]{
(a1)--[quarter left](a4) -- [quarter left](a3),
(a5) --[quarter right](a3),
(a5)--[quarter left](a1),
};
\end{feynman}

\end{tikzpicture}
\quad
\begin{tikzpicture}
\begin{feynman}

\tikzfeynmanset{every vertex={dot,minimum size=0.8mm}}
\vertex (a1);
\vertex[right=1cm of a1] (a3);

\tikzfeynmanset{every vertex={dot,minimum size=0mm}}

\vertex[right=0.5cm of a1] (a2);
\vertex[above=0.5cm of a2] (a4);
\vertex[below=0.5cm of a2] (a5);

\vertex[left=0.433cm of a2] (b1);
\vertex[left=0.433cm of a2] (b2);

\diagram*[large]{
(a1)--[quarter left](a4) -- [quarter left](a3),
(a5) --[quarter right](a3),
(a5)--[quarter left](a1),
(a1) -- (a3)
};
\end{feynman}

\end{tikzpicture}
\quad
\begin{tikzpicture}
\begin{feynman}

\tikzfeynmanset{every vertex={dot,minimum size=0.8mm}}
\vertex (a1);
\vertex[right=1cm of a1] (a3);
\vertex[right=0.5cm of a1] (a2);
\vertex[below=0.5cm of a2] (a5);

\tikzfeynmanset{every vertex={dot,minimum size=0mm}}


\vertex[above=0.5cm of a2] (a4);


\vertex[left=0.433cm of a2] (b1);
\vertex[left=0.433cm of a2] (b2);

\diagram*[large]{
(a1)--[quarter left](a4) -- [quarter left](a3),
(a5) --[quarter right](a3),
(a5)--[quarter left](a1),
(a1) -- (a3),
(a2) -- (a5),
};
\end{feynman}

\end{tikzpicture}
\end{equation}
where other topologies can be derived by setting edge powers to 0 in these topologies.

For the three topologies, the denominators momenta form a complete basis for scalar products. As a result, all scalar products in the numerator can be rewritten as raising of the powers of the denominators.

The resulting integrals with numerator 1 and various powers of the denominator can be reduced to a set of master integrals using integration-by-parts (IBP) identities~\cite{Chetyrkin:1981qh}. We use LiteRed~\cite{Lee:2012cn,Lee:2013mka} to generate a parametric reduction for each of the three topologies.
\cmtBR{TODO: one ref missing here}
The resulting 7 master integrals have been taken from the literature~\cite{Kniehl:2017ikj} with sufficiently deep expansions in $\epsilon$ for three-loop computations.
The IBP reduction and master integral computation has been verified by comparing various numerator and denominator configurations with numerical results from pySecDec~\cite{Borowka:2017idc}.

